A Survey on Annotations in Information Visualization: Empirical Insights, Applications, and Challenges

We present a comprehensive survey on the use of annotations in information visualizations, highlighting their crucial role in improving audience understanding and engagement with visual data. Our investigation encompasses empirical studies on annotations, showcasing their impact on user engagement, interaction, comprehension, and memorability across various contexts. We also study the existing tools and techniques for creating annotations and their diverse applications, enhancing the understanding of both practical and theoretical aspects of annotations in data visualization. Additionally, we identify existing research gaps and propose potential future research directions, making our survey a valuable resource for researchers, visualization designers, and practitioners by providing a thorough understanding of the application of annotations in visualization.

==> sec-intro.tex <==
\section{Introduction}
\label{sec.intro}










Annotations play a significant role in visualizations, serving as guides, providing additional context, and emphasizing critical key data features, thereby enhancing data comprehension. While there remains no consensus definition for what an annotation is (see \autoref{sec.design-space.what}), in general, they are graphical or textual elements added to an existing visualization that serves as an additional attribute for associated data items~\cite{munzner2014visualization}. 
Annotations aid in structuring the mental model of viewers when they use visualizations to understand data~\cite{cedilnik2000procedural}. Furthermore, they have been recognized as a critical task facilitating visual data analysis~\cite{heer2012interactive, zhao2016annotation}, crucial for externalizing and exploring data~\cite{kang2014character, sevastjanova2021visinreport, mahyar2012note, shrinivasan2009connecting, shrinivasan2008supporting, kim2019inking, choe2015characterizing, heer2012interactive, lin2022data, romat2019activeink, williams2023data}, aiding collaborative sensemaking~\cite{sanderson1994exploratory, chen2011supporting, chen2010click2annotate, mahyar2012note, mahyar2014supporting, isenberg2006interactive, robinson2008collaborative, kong2009perceptual, ellis2004collaborative}, and contributing to narrative storytelling~\cite{segel2010narrative, lee2015more, kosara2013storytelling, hullman2011visualization, satyanarayan2014authoring, ge2020canis, rahman2023exploring}.

\begin{figure}[!b]
  \centering
  \includegraphics[width=0.975\linewidth]{figures/papers_by_years.png} 
  \caption{The bar chart depicting the number of papers surveyed by year illustrates a noteworthy increase in publications discussing the importance, application, and tools for annotations in visualizations
  }
  \label{fig:papers_by_year}
\end{figure}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/examples/nyt-conn-scatter.pdf}
    \caption{This connected scatterplot from the New York Times depicts the correlation between oil prices and oil consumption from 1964 to 2007~\cite{10.1111/j.1740-9713.2012.00605.x}. The horizontal axis indicates global oil consumption, while the vertical axis represents oil prices. The line shifts to the right when consumption increases and prices remain stable. In contrast, the line moves upward when prices rise and consumption levels off. Significant events are annotated with text, highlighted by rectangles, and pinpointed with arrows to mark the precise point in time on the chart.}
    \label{fig:nyt-conn-scatter}
\end{figure*}




\dl{needs revision} Over the past two decades, many commercial interactive data visualization tools, such as Tableau, Microsoft PowerBI, and Google Data Studio, have emerged, supporting the annotation of visualizations and dashboards with textual and graphical elements. Notably, significant research in annotation within the visualization community has been inspired by the work of practitioners. For instance, early work by Segel et al.~\cite{segel2010narrative} explored the role of annotations in narrative visualizations, focusing on how data journalists use annotations for storytelling. Heavily annotated charts from the New York Times graphics team, such as the connected scatterplots by Amanda Cox, Hannah Fairfield, and others\cite{cox_nguyen_oil_prices_2008, fairfield_driving_reverse_2010, fairfield_driving_safety_2012} (see~\autoref{fig:nyt-conn-scatter}), have also inspired research, highlighting the importance and utility of annotations for better comprehension and clarity. Additionally, Ren et al.'s work was influenced by the New York Times' interactive chart-making tool, Mr. Chartmaker~\cite{mrchartmaker_2015}. Furthermore, publication trends over the past twenty years (see~\autoref{fig:papers_by_year}) indicate a growing interest in annotations within the visualization community. The number of research articles on annotations, including tools for authoring annotations (e.g.,~\cite{ren2017chartaccent, chen2010click2annotate}), techniques for various annotation approaches (e.g.,~\cite{cedilnik2000procedural, badam2022integrating}), and empirical studies on different aspects of annotating visualizations (e.g.,~\cite{stokes2022striking, borkin2015beyond}), has significantly increased. This trend underscores the rising recognition of annotations' importance in enhancing visual data interpretation and interaction. 



Despite the prevalent application and acknowledged importance of annotations in visualizations, there is a noticeable gap: the absence of a comprehensive survey on this topic. In response to this gap and recognizing the need for a consolidated understanding, this paper presents a systematic literature survey on annotations in visualizations that provides an overview of the annotation landscape in visualization by examining developments over the past two decades. The review covers the existing design spaces of annotations, different techniques for annotating visualizations, and the various features of tools that facilitate authoring annotations in visualizations. It also explores empirical studies highlighting different aspects of applying and using annotations in visualizations alongside their diverse applications for various purposes. Additionally, the survey discusses the challenges in this area and highlights areas that require further investigation.

\dl{remove students?} Our survey offers essential insights on the current state of annotation uses in varied contexts and future research directions, empowering a broad spectrum of individuals, from researchers and visualization designers to practitioners and students. Researchers will find it valuable for understanding the existing tools, techniques, and practices in annotation and identifying new research opportunities. Visualization designers and practitioners can leverage the insights from this survey to adopt innovative annotation techniques and best practices, enhancing their design processes and outputs. Students involved in designing or building visualization systems that facilitate annotation will find this comprehensive overview particularly beneficial, as it deepens their understanding of the subject and its practical applications.

Following the \textit{Introduction}, the paper unfolds with \textit{Section 2: Methodology}, detailing the systematic approach for literature review, analysis, and defining the survey's scope. Next, \textit{Section 3: Annotation Primer} delves into the foundational aspects of annotations, covering their definitions, types, targets, and design spaces. \textit{Section 4: Empirical Studies} then critically examines the influence of annotations across various visual contexts. \textit{Section 5: Applications and Utilities} explores the wide-ranging applications of annotations, followed by \textit{Section 6: Discussion}, which addresses existing research gaps and outlines future research directions. Finally, the paper concludes with \textit{Section 7: Conclusion}.

















==> sec-libraries.tex <==
\subsection{Annotations in Visualization Libraries}
\label{sec.libraries}















Matplotlib\cite{tosi2009matplotlib}, tailored for Python users, and ggplot2\cite{wickham2011ggplot2}, designed for the R community, both require manual coding for annotations. Matplotlib offers diverse annotation features, ideal for Python programmers seeking detailed control. ggplot2, with its layering system, allows annotations to be added without impacting the base plot, beneficial for clarity and detail in R-based visualizations.

VisDock\cite{choi2015visdock} introduces a novel approach by treating annotations as independent overlays, providing flexibility and collaborative capabilities in web-based visualizations. This method is particularly useful for interactive and shared environments. Protovis\cite{2009-protovis}, utilizing a declarative JavaScript approach, offers dynamic interaction and shared properties among marks, differing from the direct annotation methods of D3.js and Vega.


==> sec-paper-collection.tex <==
\section{Methodology}
\label{sec.paper-collection}

We plan to review the literature on annotations in visualizations from the last 20 years by constructing a corpus published in standard visualization venues that include IEEE VIS, EuroVis, ACM CHI, VAST, IEEE PacificVis, TVCG, CGF, Information Visualization, etc. Our keywords are: \textit{annotate}, \textit{annotated charts}, \textit{annotation}, and \textit{annotations in visualizations} for literature survey. Additionally, we will examine references in these articles to identify more related papers. 

Our inclusion criteria pivot on papers that offer a keen focus on detailing specific annotation methods, techniques, guidelines, use-cases, applications, and empirical studies. We will prioritize literature that not only discusses but also provides detailed explorations of at least one significant facet of annotations in visualizations, ensuring alignment with our research aims. Conversely, our exclusion criteria are designed to systematically omit papers that provide merely a casual mention of annotations without detailed analyses of specific use-cases or applications. We discard literature outside our specified publication time frame and those papers that do not offer substantive insights into our targeted aspects of annotations, along with those focusing on generalized visualization without specific annotation details. By following this method, we anticipate uncovering a vast corpus of studies on annotations in visualizations.


==> sec-relevance.tex <==
\section{Relevance to the Visualization Community}
\label{sec.relevance}

As detailed in~\autoref{sec.intro}, annotations are vital to visualizations as they enhance visual data representation, enrich the narrative, provide additional context, and emphasize critical insights. Their ability to add clarity ensures that both experts and laypersons understand complex data sets. We hope to serve two primary purposes through our proposed survey:

\begin{itemize}
    \item \textbf{Combining scattered knowledge:} We aim to provide a holistic understanding of the use of annotations in visualizations by exploring their definitions, types, techniques, and varied applications across domains. Our goal is to create a streamlined, accessible resource for those eager to grasp comprehensive annotation practices.

    \item \textbf{Finding research gaps and opportunities} Through a detailed examination of the existing literature and current practices, we strive to uncover areas yet to be investigated within visualization annotations. By emphasizing these untapped areas, we aim to chart a path for forthcoming research and novel advancements in the field.
\end{itemize}

\noindent\textbf{Target Audience}\hspace{5pt} 
Our proposed survey is intended for researchers, data journalists, data scientists, visualization practitioners, and students specializing in visualization. While researchers will dive deep into various aspects of annotations, identifying potential future research opportunities and linking past studies with emerging areas, other professionals like data journalists, data scientists, and visualization practitioners stand to benefit by enhancing their storytelling capabilities, refining visualization techniques, improving data interpretation, optimizing user engagement, adopting best practices for annotation integration, and navigating challenges for varied audiences and platforms. Overall, our proposed survey seeks to provide a robust foundation in the field while also anticipating the delivery of insights into future trends, aiming to position all our intended readers for success in their academic and professional pursuits.


==> sec-research-directions.tex <==
\section{Future Research Directions}
\label{sec.research-directions}

\begin{itemize}
    \item How much annotation do we need?~\cite{stokes2022striking, chen2023calliope}
    
\end{itemize}



==> sec-table_primer.tex <==












==> sec-taxonomy.tex <==
\section{Taxonomy}
\label{sec.taxonomy}
































































==> sec-techniques.tex <==








 





























==> sec-tools.tex <==
\section{Annotation Tools}
\label{sec.tools}









































